Knowledge Evolution in Neural Networks

Deep learning relies on the availability of a large corpus of data (labeled or unlabeled). Thus, one challenging unsettled question is: how to train a deep network on a relatively small dataset? To tackle this question, we propose an evolution-inspired training approach to boost performance on relatively small datasets. The knowledge evolution (KE) approach splits a deep network into two hypotheses: the fit-hypothesis and the reset-hypothesis. We iteratively evolve the knowledge inside the fit-hypothesis by perturbing the reset-hypothesis for multiple generations. This approach not only boosts performance, but also learns a slim network with a smaller inference cost. KE integrates seamlessly with both vanilla and residual convolutional networks. KE reduces both overfitting and the burden for data collection. We evaluate KE on various network architectures and loss functions. We evaluate KE using relatively small datasets (e.g., CUB-200) and randomly initialized deep networks. KE achieves an absolute 21% improvement margin on a state-of-the-art baseline. This performance improvement is accompanied by a relative 73% reduction in inference cost. KE achieves state-of-the-art results on classification and metric learning benchmarks. Code available at http://bit.ly/3uLgwYb

==> conv_popup.tex <==
\subsection{Conv-popup}\label{sec:conv_popup}
We briefly reviews the edge-popup algorithm before introducing our conv-popup.
\begin{figure}[t]
	\centering
	\scriptsize
	\includegraphics[width=0.9\linewidth]{figures/edge_popup}
	\caption{Edge-popup illustration using a toy neurons $v$ with a single incoming edge from a neuron $u$.}
	\label{fig:edge_popup}
	% A $4\times4$ filter $f$ is employed for visualization purpose. 
\end{figure}

\heading{Edge-popup Algorithm}

%, each layer has $W_l\in R^{|W_l|}$ where $|W_l|$ is the number of weights in layer $l$. Given a dense network $N$, 

We first introduce our mathematical notation. Given a neural network $N$ with weight $W$ and bias $B$ parameters, we assume a network has $L$ layers and. The edge-popup works on a weight-level granularity. Thus for a neuron $v$, the input and output are denoted by $v_i$ and $v_o$, respectively. The neuron's output $v_o=\sigma(v_i)$ for a non-linear activation function $\sigma$ (\eg ReLU~\cite{krizhevsky2012imagenet}). For a neuron $v$ is at layer $l$, $v_i=\sum_{u\in U}{w_{uv}u_o}$, where $U$ is the set of all neurons at layer $l-1$. The weight $w_{uv}$ can be regarded as an edge connecting the two neurons ($u,v$) as shown in~\autoref{fig:edge_popup}.

The edge-popup algorithm~\cite{ramanujan2020s} identifies an effective subnetwork $\tau$, inside $N$, by introducing popup scores $s$. For every edge $w_{uv}$, edge-popup associates a real-valued popup score $s_{uv}$. For every layer $l$ in $N$,  edge-popup identifies the subnetwork $\tau$ by selecting the edges (weights) which have the top-$k\%$ highest scores. Accordingly, the input for a neuron $v$ can be written equivalently $v_i=\sum_{u\in U}{w_{uv} u_o h(s_{uv})}$ where $h(s_uv) = 1$ if $s_uv$ is among the top $k\%$ highest scores in layer $l$ and $h(s_uv) = 0$ otherwise.

While fixing the weights $w$ of the network $N$, the edge-popup algorithm leverages  stochastic gradient descent with to optimize the popup scores $s$ as follows
\begin{equation}
s_{uv} \leftarrow s_{uv} - lr \frac{\partial L}{ \partial  v_i}u_o w_{uv},
\end{equation}
where $lr$ is the learning rate and $L$ is a loss function. After optimizing $s$, the top-$k\%$ highest scores provide a mask, in every layer $l$, that identifies the subnetwork $\tau$.

Ramanujan~\cite{ramanujan2020s} present edge-popup to find the best hypothesis within a randomly initialized network. However, edge-popup is also a pruning approach with pros and cons. For instance, edge-popup supports a large spectrum of the network architectures and loss functions. In addition, It does not introduce a regularization term. Thus, it has no hyperparameters expect the keep rate $k$. On the other hand, the limitation of edge-popup is that it always produce a dense network. Even if we naively associate a popup score to every weight parameter inside a convolutional layer, we would still require sparse BLAS libraries or even specialized hardware~\cite{han2016eie}. To tackle this limitation, we propose conv-popup.

\heading{Conv-popup Algorithm}

\begin{figure}[t]
	\centering
	\scriptsize
	\includegraphics[width=1.0\linewidth]{figures/conv_popup}
	\caption{Conv-popup illustration using a 2D convolutional filter $F \in R^{C_o \times \kappa \times \kappa \times C_i}$. In this example, the input feature map $M_l$ (right) at layer $l$ has $C_i=3$ channels and the output map $M_{l+1}$ (left) has $C_o=4$ channels . The $\circ$ and $\ast$ denote the convolution and broadcasting operations, respectively.}
	\label{fig:conv_popup}
	% A $4\times4$ filter $f$ is employed for visualization purpose. 
\end{figure}
%Similar to~\cite{liu2017learning}, we work on a convolutional filter-level, while they work on channel-level. but without the hyperparameter $\lambda$. Since we sort the scores, there is no need for the sparsity constraint. Our approach does not require a batch-norm layers. conv-popup is independent of the task-mask approach. It can be used out-of-the-box for pruning a network. By using conv-popup during training, it eliminates the need for fine-tuning (retraining) after pruning. This leads into a one-shot pruning approach that saves re-training time if pruning is the ultimate goal. 

\autoref{fig:conv_popup} illustrates the conv-popup approach using a convolutional filter $F_l\in R^{C_o\times \kappa\times \kappa \times C_i}$ at layer $l$ with multiple 2D kernels $\pi \in R^{\kappa\times \kappa }$. $C_o$ and $C_i$ denote the number of output and input channels, while $W$ and $H$ denote the feature maps' spatial dimensions. We formulate the standard convolution operation as follows
%input and output feature maps' relation is formulated as follow
\begin{equation}\label{eq:vanilla_conv}
{ M}^j_{ l+1 } = F^j_l \circ M_l,
\end{equation}
where $M_l$ is the feature map at layer $l$, $j \in \{1,..,C_o\}$ and $\circ$ denotes the convolution operation. Conv-popup associates a popup score to each individual convolutional filter,~\ie $s_l \in R^{C_o}$. Given a keep rate $k$, conv-popup selects the filters which have the top-$k\%$ highest scores. Accordingly, we rewrite the convolutional operation as follows
\begin{equation}
{ M }^j_{ l+1 } = \left(h( { s }^j_{ l })  F^j_l\right) \circ M_l,
\end{equation}
where $h({ s }^j_{ l })$ denotes the binary scalar $\{0,1\}$ corresponding to the $j^{th}$ convolutional filter. $h(s^j_l) = 1$ if $s^j_l$ belongs to the top $k\%$ highest conv-popup scores in layer $l$ and $h(s^j_l) = 0$ otherwise. The gradient of $h$ is 0 everywhere, so it is not possible to directly compute the gradient of the loss with respect to $s^j_l$. Similar to edge-popup, We use the straight-through gradient estimator~\cite{bengio2013estimating} that treats $h$ as the identity in the backwards pass -- the gradient goes ``straight-through'' $h$. Accordingly, the score at layer $l$ for a $j^{th}$ output channel is updated as follows
\begin{equation}
{ s }_{ l }^{ j }\leftarrow { s }_{ l }^{ j }-lr \sum _{ w=1 }^{ W }{ \sum _{ h=1 }^{ H }{\frac { \partial L }{ \partial { M }_{ l+1 }^{ w,h,j }}} { M }^{w,h,j}_{ l+1 }},
\end{equation}
basically, the gradient of  $h(s^j_l)$ back-propagates through all weights inside the filter $F^j_l$ for every pixel ($W \times H$) for all $C_i$ input channels (the values inside the output feature map $M_{l+1}$). Given the fit-hypothesis $H^\triangle \leftarrow h(S)$, conv-popup can extract the corresponding slim network from a vanilla CNN (VGG  and AlexNet) in a straightforward manner. However, there are multiple ways, with different degrees of complexity, to extract slim networks using conv-popup from modern networks with residual link. In the supplementary material, we propose a simple technique to prune residual networks with conv-popup.

%we expand this equation with in the appendix. 

The edge-popup and conv-popup algorithms support a large spectrum of neural networks.  However, due to its larger masking granularity, conv-popup suffers if applied to a randomly initialized neural networks (generation zero -- G0). After training  the network (G1), the fit-hypothesis identified by conv-popup significantly lags behind the fit-hypothesis  identified by edge-popup. However, if we alternate between the task and mask phases for multiple generations, the performance gap between both hypotheses closes. The next section presents the task-mask (TM) training approach. TM evaluates and refines hypotheses across generations. If a hypothesis $H^\triangledown$ is found useless, it is declared dead and a succeeding hypothesis is appointed.

% to close this performance gap, while most importantly 



==> hypotheses_ham_metric.tex <==
\subsection{Hypotheses Hamming Distance (H2D)}\label{sec:hypotheses_ham_metric}
In this section, we propose a quantitative metric to monitor hypotheses development across TM's generation. The mask phase delivers both a sparse network and a binary mask $h(S)$. We leverage hamming distance to quantify distance between hypotheses,~\ie Hypotheses Hamming Distance (H2D). In our experiments, we use S-H2D to measure \underline{s}tride between consecutive hypotheses and C-H2D to measure the \underline{c}umulative distances starting from the first mask.

% The S-H2D measures the \textbf{s}tripe between consecutive generations, while C-H2D measures the cumulative total distance traveled 


let $h(S^g_l)$ denotes the binary mask at layer $l$ after going through the mask-phase of the $g^{th}$ generations. For $g\ge2$, we formulate S-H2D and C-H2D as follows
\begin{align}
	\text{S-H2D}(g) &= { \|  h(S^{g-1}_l) , h(S^{g}_l) \|  }_{ h } \\
		\text{C-H2D}(g) &= { \|  h(S^{1}_l) , h(S^{g}_l) \|  }_{ h },
\end{align}
where ${ \|u,v  \|  }_{ h }$ is the number of places where $u\in\{0,1\}^d$ and $v\in\{0,1\}^d$ differ, normalized by the dimension $d$. Assuming a convolutional layer and a keep rate $k=0.5$, the binary mask $h(S^g_l)\in \{0,1\}^{C_o}$ will have $\frac{C_o}{2}$ zeros and $\frac{C_o}{2}$ ones. Thus, the H2D range is maximum ($\in [0,1]$) when the keep rate $k=0.5$. This range decreases as the keep rate moves away from $k=0.5$. Our experiments show that S-H2D decreases as the number of generation increases, while C-H2D increases before reaching a plateau. When C-H2D plateaus, the network's performance plateaus as well. Thus, H2D servers a termination criteria.
% if a validation split is not available.

==> mask_ham_metric.tex <==
\part{\subsection{Mask-Ham Distance Metric}\label{sec:mask_ham_metric}}

==> old_supp_mat.tex <==
The following appendix sections extend their corresponding sections in the main paper. For instance, the related-work appendix~\ref{sec:app_related} extends the related-work section in the main paper.

\appendix

%\section{Further Comments}
\section{Appendix: Related Work}\label{sec:app_related}
\begin{enumerate}
	\item Lottery Ticket hypothesis literature~\cite{frankle2018lottery,zhou2019deconstructing,frankle2019stabilizing}. Both~\cite{frankle2018lottery,zhou2019deconstructing} study the lottery ticket hypothesis on small datasets. In this literature,  the lottery ticket subnetwork is always reset to its randomly initialized weights -- $W$ at iteration zero. Frankle~\etal~\cite{frankle2019stabilizing} showed that this strict weight resetting harms performance on large scale datasets. Accordingly, weight rewinding~\cite{frankle2019stabilizing} is proposed, which 
	rewinds pruned subnetwork's weights to their former values at iteration $k$ rather than resetting them to iteration zero.
	These three papers~\cite{frankle2018lottery,zhou2019deconstructing,frankle2019stabilizing} are solving a network pruning problem. Thus, the pruned network performance is always less than or equal to the dense network. This is not the case for Task-Mask. 
	
	%\item Supermask literature~\cite{wortsman2020supermasks,ramanujan2020s}
	%\item Network initialization literature~\cite{glorot2010understanding,krahenbuhl2015data} initializes each layer independently.
	
%	\item Born again neural networks~\cite{furlanello2018born} assume a teacher model with access to a large corps of data, Task-Mask does not. In born-again, every student uses the predictions of the previous teacher model to distill knowledge, Task-Mask does not. In born-again, students are randomly initialized, Task-Mask does not.
	%	\item Our work can be regarded a a generalization of the Dense-Sparse-Dense (DSD) training protocol~\cite{han2016dsd}. Yet, there are technical and non-technical factors that differentiate our work. The technical factors are clear; 
	
	%\item SOTA on small datasets~\cite{yun2020regularizing}. Baselines: AdaCos~\cite{zhang2019adacos}, Virtual-softmax~\cite{chen2018virtual}, Maximum-entropy~\cite{dubey2018maximum,pereyra2017regularizing}, Label-smoothing~\cite{muller2019does,szegedy2016rethinking} , DDGSD~\cite{xu2019data}, BYOT~\cite{zhang2019your}
	%\item The argument that pre-trained networks~\cite{erhan2010does} and knowledge distillation~\cite{yuan2020revisiting} are just regularizers. Similarly, Task-Mask can be regarded as a weight-regularizer.
	%\item Few-show learning approaches~\cite{bateni2020improved,requeima2019fast} count on pretrained ImageNet weights~\cite{deng2009imagenet}, Task-Mask do not.
	%\item I should cite some evolutionary machine learning literature.
\end{enumerate}

\section{Appendix: Approach}
\begin{equation}
{ M }_{ l+1 }^{ w,h,j }=\sum _{ i=1 }^{ C_{ i } }{ \sum _{ c=1 }^{ \kappa  }{ \sum _{ r=1 }^{ \kappa  }{ 
			{ w }_{ ji }^{ (c,r) }{ M }_{ l }^{ \left( w+c-\left\lceil \frac { \kappa  }{ 2 }  \right\rceil ,h+r-\left\lceil \frac { \kappa  }{ 2 }  \right\rceil ,i \right)  } 
}  }  } 
\end{equation}
%where $\Psi_i  = { w }_{ ji }^{ (c,r) }{ M }_{ l }^{ \left( w+c-\left\lceil \frac { \kappa  }{ 2 }  \right\rceil ,h+r-\left\lceil \frac { \kappa  }{ 2 }  \right\rceil ,i \right)  } $


\begin{equation}
{ M }_{ l+1 }^{ w,h,j }=\sum _{ i=1 }^{ C_{ i } }{ \sum _{ c=1 }^{ \kappa  }{ \sum _{ r=1 }^{ \kappa  }{ { w }_{ ji }^{ (c,r) }{ M }_{ l }^{ \left( w+c-\left\lceil \frac { \kappa  }{ 2 }  \right\rceil ,h+r-\left\lceil \frac { \kappa  }{ 2 }  \right\rceil ,i \right)  } }  } h\left( { s }_{ l }^{ j } \right)  } 
\end{equation}

\begin{equation}
{ s }_{ l }^{ j }\leftarrow { s }_{ l }^{ j }-lr\sum _{ i=1 }^{ C_{ i } }{ \sum _{ w=1 }^{ W }{ \sum _{ h=1 }^{ H }{ \sum _{ c=1 }^{ \kappa  }{ \sum _{ r=1 }^{ \kappa  }{ \frac { \partial L }{ \partial { M }_{ l+1 }^{ w,h,j } } { w }_{ ji }^{ (c,r) }{ M }_{ l }^{ \left( w+c-\left\lceil \frac { \kappa  }{ 2 }  \right\rceil ,h+r-\left\lceil \frac { \kappa  }{ 2 }  \right\rceil ,i \right)  } }  }  }  }  } 
\end{equation}


\begin{figure*}
	\centering
	\includegraphics[width=1.0\linewidth]{figures/simple_pruning}
	\caption{A simple approach to convert a toy residual network into a slim residual network. We prune the output filters and the corresponding input channels highlighted in green. We omit the RELU and batch norm layers for brevity; However, they will be pruned as well. This simple approach will keep a lot of filters set to zero, to  add feature maps properly. Yet, the computational reduction during inference remains significant.}
	\label{fig:simplepruning}
\end{figure*}


\section{Appendix:  Experiments}

\heading{TM vs RePr:} In the paper, we highlight two differences between TM and RePr. Yet, there are other worth nothing differences. (\rom{1}) TM uses popup scores to quantify each filter's importance. Our ablation study (Figure~\ref{}) emphasizes the importance of \textbf{re-using} these scores across different mask phases. Basically, TM is biased towards filters (hypotheses) that survived previous mask phases. This achieves superior performance, compared to resetting the scores and re-ranking filters from scratch. However, RePr ranks filters from scratch at every pruning stage. This is an inferior ranking policy.

(\rom{2}) RePr and TM also differ in terms of the final network sparsity. Since RePr is a training approach for large datasets, RePr terminates with a dense network. In contrast, TM is a training approach for small datasets. Thus, TM is able to deliver both a sparse and dense networks (Figure~\ref{}) due to the redundancy in deep networks' trained on small datasets.

%For example, If the probably of a filter being redundant is $p$ at the first pruning stage, 
 
% does not have an equivalent 



\subsection{Interesting Ablation Studies}
I am looking forward to the following set of experiments

\begin{enumerate}
	\item Can the knowledge accumulated from a single dataset transfer to a different dataset? For instance, If I train 100 generations on Flower102, how do these generations perform on CUB-200?
	\item Apply Task-Mask on feature embedding networks. To my knowledge, Task-Mask would be the first approach  that boosts \textit{both} classification and feature embedding networks on small datasets.
	\item How do the filters of the first conv layer look like? When pretrained on ImageNet, the filters of the first conv layer look like edge detectors. Can Task-Mask learn similar filters from a small dataset? This would be a sign for generalization beyond the small dataset used during evolution.
	\item In this paper, I am going to focus on supervised tasks only. However, investigation on unsupervised tasks is an interesting future extension. 
	
	\item Typical regularization approaches fail as the trained network becomes deeper. Task-Mask approach fails if and only if the dataset gets bigger while the network size remains fixed or decreases. As the network-size gets bigger, task-mask should remain competitive. Assuming a fixed pruning rate, as the network becomes bigger, the number of possible subnetworks increases. The Mask-phase, having a large diversity in weights, will locate better fit-weights which speed up the performance progress. 
	
	%However, it is the opposite for Task-Mask.  
\end{enumerate}

The following is a set of ablation studies that I am *not* looking for, but I should do

\begin{enumerate}
	\item Does a better sampling distribution $D$ exist? I expect a sampling strategy that takes the weight magnitude into account to be better~\cite{zhou2019deconstructing}. However, the anticipated improvement will not justify the added complexity. 
	\item The reason I am not identifying fit-bias is that (1) I do not think bias terms correlate across layers, (2) the bias term reflects how a network favors or thwarts classes against each other.  Bias is a way to define a threshold between classes, it reflects the distribution of the input classes; majority classes have bigger bias terms while minority classes have a smaller bias. Accordingly, there is no bad and fit-bias to transfer. I should show empirically that transfer fit-bias brings no improvement.
\end{enumerate}



\subsection{Misc Notes}
\begin{enumerate}
	\item The \textit{current} main limitation of Task-Mask is the computational complexity during training. For a single dataset, the \textit{current} Task-Mask approach trains $2 \times G$ neural networks,~\ie $G$ tasks and $G$ masks networks. At this preliminary stage, I intentionally did not pay attention to this issue because I wanted to focus more on the approach and the SOTA performance even if it is computationally costly. It is important to note that one epoch of ImageNet is computationally equivalent to one thousand epochs of Flower102. I am not promising anything, but I will think about how to reduce the training cost in the upcoming stage. 
	% For a small dataset, this is not a huge issue. 
	
	\item There is an expected argument that this approach is not valuable for big datasets. While this argument is expected, I think it is a shortsighted one. In less than a decade, the size of neural networks will grow very big~\cite{brown2020language}. If ImageNet is currently enough to train a deep network, it won't be in the future -- it will become a toy dataset. Of course, self/un-supervised approaches do not need labels, yet they need a ton of unlabeled data. This is not a feasible solution for applications such as autonomous navigation, medical imaging, and any application with privacy concerns. 
	
	\item The killing argument is, why not use ImageNet weights, instead of random weights? The best reply is to show that Task-Mask boosts the performance of networks initialized with either random or ImageNet weights. Maybe it will, I am not sure! More experiments are needed to address this argument.
	
	%I think it is better if I presented Task-Mask not as an approach for small datasets, but as an approach for labeled datasets on very deep neural networks. But, I can not train any very deep neural network on vulcan!
	
	\item Task-Mask integrates seamlessly with all neural network training tricks.  I should capitalize on this strength in my experiments. For example, I am currently using cross entropy with the label smoothing regularizer, but I can also use the SOTA class-wise regularizer~\cite{yun2020regularizing}.
	
	
	% I a presented Task-Mask approach as a solution to train a relatively deep network on a relatively small tasks -- not an absolute small.
\end{enumerate}

\begin{table}[]
	\scriptsize
	\begin{tabular}{lll}
		\toprule
		Layers                & Dense  $N$                       & Fit-hypothesis $H^\triangle$ ($s_r=0.5$)          \\
		
		\midrule
		conv1                             & 64 $\times$ 7 $\times$ 7 $\times$ 3    & 32 $\times$ 7 $\times$ 7 $\times$ 3    \\
		bn1                               & 64                                     & 32                                     \\
		layer1.0.conv1                    & 64 $\times$ 3 $\times$ 3 $\times$ 64   & 32 $\times$ 3 $\times$ 3 $\times$ 32   \\
		layer1.0.bn1                      & 64                                     & 32                                     \\
		layer1.0.conv2                    & 64 $\times$ 3 $\times$ 3 $\times$ 64   & 32 $\times$ 3 $\times$ 3 $\times$ 32   \\
		layer1.0.bn2                      & 64                                     & 32                                     \\
		layer1.1.conv1                    & 64 $\times$ 3 $\times$ 3 $\times$ 64   & 32 $\times$ 3 $\times$ 3 $\times$ 32   \\
		layer1.1.bn1                      & 64                                     & 32                                     \\
		layer1.1.conv2                    & 64 $\times$ 3 $\times$ 3 $\times$ 64   & 32 $\times$ 3 $\times$ 3 $\times$ 32   \\
		layer1.1.bn2                      & 64                                     & 32                                     \\
		layer2.0.conv1                    & 128 $\times$ 3 $\times$ 3 $\times$ 64  & 64 $\times$ 3 $\times$ 3 $\times$ 32   \\
		layer2.0.bn1                      & 128                                    & 64                                     \\
		layer2.0.conv2                    & 128 $\times$ 3 $\times$ 3 $\times$ 128 & 64 $\times$ 3 $\times$ 3 $\times$ 64   \\
		layer2.0.bn2                      & 128                                    & 64                                     \\
		layer2.0.downsample.0             & 128 $\times$ 1 $\times$ 1 $\times$ 64  & 64 $\times$ 1 $\times$ 1 $\times$ 32   \\
		layer2.0.downsample.1             & 128                                    & 64                                     \\
		layer2.1.conv1                    & 128 $\times$ 3 $\times$ 3 $\times$ 128 & 64 $\times$ 3 $\times$ 3 $\times$ 64   \\
		layer2.1.bn1                      & 128                                    & 64                                     \\
		layer2.1.conv2                    & 128 $\times$ 3 $\times$ 3 $\times$ 128 & 64 $\times$ 3 $\times$ 3 $\times$ 64   \\
		layer2.1.bn2                      & 128                                    & 64                                     \\
		layer3.0.conv1                    & 256 $\times$ 3 $\times$ 3 $\times$ 128 & 128 $\times$ 3 $\times$ 3 $\times$ 64  \\
		layer3.0.bn1                      & 256                                    & 128                                    \\
		layer3.0.conv2                    & 256 $\times$ 3 $\times$ 3 $\times$ 256 & 128 $\times$ 3 $\times$ 3 $\times$ 128 \\
		layer3.0.bn2                      & 256                                    & 128                                    \\
		layer3.0.downsample.0             & 256 $\times$ 1 $\times$ 1 $\times$ 128 & 128 $\times$ 1 $\times$ 1 $\times$ 64  \\
		layer3.0.downsample.1             & 256                                    & 128                                    \\
		layer3.1.conv1                    & 256 $\times$ 3 $\times$ 3 $\times$ 256 & 128 $\times$ 3 $\times$ 3 $\times$ 128 \\
		layer3.1.bn1                      & 256                                    & 128                                    \\
		layer3.1.conv2                    & 256 $\times$ 3 $\times$ 3 $\times$ 256 & 128 $\times$ 3 $\times$ 3 $\times$ 128 \\
		layer3.1.bn2                      & 256                                    & 128                                    \\
		layer4.0.conv1                    & 512 $\times$ 3 $\times$ 3 $\times$ 256 & 256 $\times$ 3 $\times$ 3 $\times$ 128 \\
		layer4.0.bn1                      & 512                                    & 256                                    \\
		layer4.0.conv2                    & 512 $\times$ 3 $\times$ 3 $\times$ 512 & 256 $\times$ 3 $\times$ 3 $\times$ 256 \\
		layer4.0.bn2                      & 512                                    & 256                                    \\
		layer4.0.downsample.0             & 512 $\times$ 1 $\times$ 1 $\times$ 256 & 256 $\times$ 1 $\times$ 1 $\times$ 128 \\
		layer4.0.downsample.1             & 512                                    & 256                                    \\
		layer4.1.conv1                    & 512 $\times$ 3 $\times$ 3 $\times$ 512 & 256 $\times$ 3 $\times$ 3 $\times$ 256 \\
		layer4.1.bn1                      & 512                                    & 256                                    \\
		layer4.1.conv2                    & 512 $\times$ 3 $\times$ 3 $\times$ 512 & 256 $\times$ 3 $\times$ 3 $\times$ 256 \\
		layer4.1.bn2                      & 512                                    & 256                                    \\
		fc                                & 102 $\times$ 512                       & 102 $\times$ 256                       \\
		\midrule
		\midrule
		\#Ops (GOps) & 3.632420  &  0.968436 \\
		\#Parameters (M) & 11.285862 &  2.853606 \\
		\bottomrule
	\end{tabular}
\end{table}

==> related_work__Ahmed_Taha_s_conflicted_copy_2020-11-07_.tex <==
\section{Related Work}\label{sec:related_work}
This section compares knowledge evolution (KE) with two prominent training approaches: Born-Again Networks (BANs)~\cite{furlanello2018born} and  Dense-Sparse-Dense (DSD)~\cite{han2016dsd}. In the paper appendix, we compare KELS with the pruning literature~\cite{lecun1990optimal,hassibi1993second,han2015learning,han2015deep,li2016pruning,wen2016learning,zhou2016less,luo2017thinet,liu2017learning,yu2018nisp,huang2018condensenet}

%~\cite{han2015deep,han2015learning,li2016pruning,wen2016learning,liu2017learning,huang2018condensenet,yu2018nisp}.
% and present Task-Mask as a regularization technique.

%Since the gradient of $h$ is 0 everywhere it is not possible to directly compute the gradient of the loss with respect to $s_uv$. We instead use the straight-through gradient estimator~\cite{bengio2013estimating}, in which h is treated as the identity in the backwards pass – the gradient goes “straight-through” h. Consequently, we approximate the gradient to suv a



DSD~\cite{han2016dsd} starts with a dense-phase to learn connections' weights and importance. The sparse-phase prunes the unimportant connections  and re-trains the network given a sparsity constraint. The final dense-phase removes the sparsity constraint, re-initializes the pruned connections,  and retrains the entire dense network. KE differs from DSD in multiple ways: (1) DSD masks (prunes) individual weights, while KE masks complete convolution kernels. Thus, DSD delivers dense networks, while KE delivers both dense and slim networks. (2) KE introduces the idea of a fit-hypothesis that encapsulates a network's knowledge, then transfer this knowledge across generations to boost performance.

%, and .

% , equipped with our splitting technique,

% (1) DSD stops after the second generation, while TM shows the benefit of repeating this process for multiple generations.

%Our experiments explain why zero-resetting individual weights worked for DSD, but this re-initialization is inferior when working with convolutional filters.

BANs~\cite{furlanello2018born} is a knowledge-distillation based approach. Similar to KE, BANs re-trains the same architecture iteratively. However, to transfer knowledge between successive networks, BANs use the class-logits distribution, while KE uses the networks' weights. This explains why BANs use the teacher-student terminology while KE uses the parent-sibling terminology. This difference is important because (1) training a teacher network, which teaches future students, requires a large corpus of data (labeled or not). In contrast, KE acknowledges the deficiency of a parent network trained on a small dataset; (2) BANs randomly initialize student networks while KE utilize the knowledge of a  parent network to initialize the next generation.

%assume a teacher model with access to a large corps of data, Task-Mask does not. In born-again, every student uses the predictions of the previous teacher model to distill knowledge, Task-Mask does not. In born-again, students are randomly initialized, Task-Mask does not.


We distance our work from neural architecture search (NAS) literature~\cite{zoph2016neural,liu2018progressive} such as Neural Rejuvenation~\cite{qiao2019neural} and MorphNet~\cite{gordon2018morphnet}. We assume the network's connections and the number of parameters are fixed.

%  In the supplementary material, we show how Task-Mask can be regarded as a regularization technique. This follows recent literature that regards pretrained networks, knowledge distillation~\cite{hinton2015distilling} and label smoothing~\cite{szegedy2016rethinking} as regularization techniques~\cite{erhan2010does,yuan2020revisiting,muller2019does} respectively.




==> split_network_intuitions.tex <==
\subsection{The Split-Networks Intuitions}



==> task_mask_approach.tex <==
\subsection{The Task-Mask Approach}\label{sec:task_mask_approach}
At a high level, given a network $N$ containing a set of hypotheses $H$ (subnetworks), the task phase nudges these hypotheses to minimize an objective function. Later, the mask-phase splits $H$ into fit $H^\triangle$ and dead $H^\triangledown $ hypotheses. The hypothesis $H^\triangledown $ is declared dead, reinitialized and merged with $H^\triangle$ before re-entering the task-phase.

\heading{Task Phase}

We evaluate our approach using two supervised tasks: (1) classification and (2) metric learning. The performance of deep networks on small datasets is intensively studied using the classification task~\cite{szegedy2016rethinking,pereyra2017regularizing,dubey2018maximum,chen2018virtual,muller2019does,xu2019data,zhang2019your,zhang2019adacos,yun2020regularizing}. Thus, the classification task provides a rigorous quantitative benchmark.  The metric learning evaluation highlights the flexibility of our approach and distances the Task-Mask approach from the mainstream literature that requires class logits.

We denote $x \in X$ as input and $y \in Y = \left\{1, ..., C\right\}$ as its ground-truth label. This notation is used to present both the softmax and triplet losses. These two loss functions are chosen because most supervised tasks employ one of them. 

\noindent\textbf{Cross-Entropy Loss:}
The cross-entropy loss for a classification network $N$ is formulated as follows
%A classification network $N$ model a posterior predictive distribution as follows
\begin{equation}
	CE_{(x,y)} = -log \frac{exp\left(N(x;y)\right)}{\sum^C_{i=1}{ exp\left(N(x;i)\right) }}
\end{equation}
where $N(x;y)$ denotes the output logit for class $y$.
% and $t > 0$ is the temperature parameter.

\noindent\textbf{Triplet Loss:} A metric learning network learns an embedding where samples from the same class are pulled together, while samples from different classes are pushing apart. Triplet loss is a simple and efficient ranking loss used to train feature embedding networks; it is defined as follows
% 
\begin{equation}\label{eq:triplet}
\text{TL}_{(a,p,n) \in T} ={ { \left[  { (D_{a,p}-{ D_{a,n} } +m) }  \right]  }_{ + }  }
\end{equation}
where ${ \left[ \sbullet[0.75] \right]  }_{ + }= max(0,\sbullet[0.75])$, $m$ is the margin between classes.  $D_{x_1,x_2}=D(N(x_1),N(x_2))$; $N(\sbullet[0.75]) $ and $D(,)$ are the embedding and Euclidean distance functions, respectively. In~\autoref{eq:triplet}, $a$, $p$, and $n$ are the anchor, positive, and negative images in a single triplet $(a,p,n)$ from the triplets set $T$. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.4\linewidth]{figures/hard_semi_negative}
	\caption{Triplet loss tuple (anchor, positive, negative) and margin $m$. The (h)ard, (s)emi-hard and (e)asy negatives are highlighted in black, gray and white, respectively.}
	\label{fig:semi_neg}
\end{figure}


\begin{equation}\label{eq:btl_semi_neg}
D_{a,p} < D_{a,n} < D_{a,p} + m,
\end{equation}

The performance of triplet loss relies heavily on the sampling strategy. Since we are training randomly initialized networks, We leverage semi-hard sampling~\cite{schroff2015facenet} for its stability. In semi-hard negative sampling, instead of picking the hardest positive-negative samples, all anchor-positive pairs and their corresponding semi-hard negatives are considered. Semi-hard negatives are further away from the anchor than the positive exemplar yet within the banned margin $m$ as shown in~\autoref{fig:semi_neg}. Semi-hard negatives ($n$) satisfy~\autoref{eq:btl_semi_neg}

% the weights $W_l$ of layer $l$ are no longer random. 
\textbf{After the task-phase}, the mask-phase identifies the fit-hypothesis $H^\triangle$. Once identified, $H^\triangle$ will be used to re-initialize the next network generation before re-entering the task-phase.

%Our formulation does not make any assumption about the network architecture, loss function or the output dimensionality.



\heading{Mask Phase}

\noindent\textbf{Identify fit-hypothesis $H^ \triangle$:} Given a randomly initialized network $N$, Zhou~\etal~\cite{zhou2019deconstructing} coined the term \textit{supermask} – a subnetwork of a
randomly initialized neural network that achieves high accuracy without training. Ramanujan~\etal~\cite{ramanujan2020s} follow up by proposing an efficient algorithm to find this supermask. In previous literature~\cite{zhou2019deconstructing,ramanujan2020s,wortsman2020supermasks}, the supermask served as a \textit{randomly initialized} pruned network. In contrast, we leverage conv-popup to identify the fit-hypothesis $H^\triangle$ inside a \textit{trained} network. While previous literature~\cite{zhou2019deconstructing,ramanujan2020s,wortsman2020supermasks} delivers a sparse network, conv-popup delivers a slim network. Both sparse and slim networks have a large number of zero weights. Yet, a sparse network requires a special libraries or hardware to perform efficiently. In contrast, a slim network performs efficiently without special handling,~\ie zero-weights are simply trimmed.

Traditional weight initialization approaches~\cite{glorot2010understanding,krahenbuhl2015data} initialize layers' weights independently. In contrast, $H^\triangle$ entangles the networks' weights $W$ (and convolutional-filters $F$) across the network's layers. In~\autoref{fig:overview}, we illustrate this idea using the edges' colors and how we take advantage of this cross-layer dependency to re-initialize the network. This insight guides how we transfer $H^ \star$ to the next network generation.

%The fit-hypothesis $H^\triangle$ captures the network essence. One key insight about $H^\triangle$ is that It entangles the networks' weights $W$ (and convolutional-filters $F$) across the network's layers.  I

%The mask $S^T$ identifies the fit-weights $W ^ \star \subset W$ that capture the network essence (performance). One key insight about $W^ \star_l$ is that these weights are entangled across the network's layers. Unlike traditional weight initialization approaches, where every layer's weights are independently initialized, the fit-weights in layer $l$, $W^ \star_l$, are tightly dependent on the fit-weights of the preceding $W^ \star_{l-1}$ and succeeding $W^ \star_{l+1}$ layers. In~\autoref{fig:overview}, we illustrate this idea using the edges' colors and how we take advantage of this cross-layer dependency to re-initialize the network. This insight guides how we transfer $W^ \star$ to the next network generation. 

%Our proposed knowledge transfer approach is most importantly about how the weights are connected across layer.

\noindent\textbf{Transfer fit-hypothesis $H^ \triangle$:} We propose a simple, yet efficient, technique to transfer fit-hypothesis $H^ \triangle$ and replace the dead hypothesis $H^\triangledown$ across the network's generations. We illustrate our technique using a single convolutional layer, and repeat this technique for every layer. The proposed technique makes no assumption about the layer type. Thus, it supports fully connected, graph convolution and recurrent layers.

The popup scores $h(S)$ defines the fit-hypothesis $H^\triangle$. For a given convolutional layer $l$, $h(S_l)\in \{0,1\}^{C_o}$ and $h(s^j_l) = 1$ if $s^j_l$ belongs to the top $k\%$ highest conv-popup scores in layer $l$ and $h(s^j_l) = 0$ otherwise. We re-initialize $F_l$ using the previous generation's weights as follows
\begin{equation}\label{eq:transfer_fit_hypothesis}
	F_l = h(S_l) \ast F_l  + \left(1-h(S_l)\right)  \ast T_r,
\end{equation}
where $\ast$ denotes the broadcasting operation and $T_r$ is a randomly initialized tensor. $T_r$ and $F_l$ have the same size,~\ie $T_r\in R^{C_o \times \kappa \times \kappa \times C_i}$. $T_r$ is initialized using the default initialization distribution. For example, PyTorch use kaiming uniform~\cite{he_delving_2015} for convolution layers. Fully connected layer can be initialized similarly by replacing $F_l$ with $W_l/B_I$ and using their corresponding popup scores.


Initially, all network parameters (weights $W$, bias $B$, convolutional filters $F$, batch norm $BN$ and popup scores $S$) are initialized randomly. The task-phases update the $W$, $B$, $BN$, and $F$, but not $S$.  The mask phases keep $W$, $F$, and $BN$ frozen and update $S$ only to find the fit-hypothesis $H^\triangle$. Before re-entering task-phase, ~\autoref{eq:transfer_fit_hypothesis} re-initializes $W$, $F$, and $B$. The batch norm parameters $BN$ transfer as it is between task-phases,~\ie there is no popup scores for $BN$. Similarly, $S$ transfers as it is between mask-phases. Our experiments show that transferring the popup scores $S$ between mask-phases leads to better performance compared to re-initializing $S$ randomly before every mask-phase.\autoref{Algo:task_mask} summarizes Task-Mask approach.

% To slim a batch norm layer, we use the popup score of the preceding layer.

% =\left[w_1,...,w_p\right]
%  with $W_l\in R^p$ and a supermask $S^T_l =\left\{0,1\right\}^p$  

%After training a network on a task $T$ and identifying the supermask $S^T$, a network layer $l$ has a $W^ \star_l =\left[w^\star_1,...,w^\star_k\right] \subset W_l$. $W^ \star_l$ is a subset of $W_l$ identified by  $S^T_l\in\left\{0,1\right\}^{|W_l|}$. This subset contains $k$ weights where   $k$ depends on the pruning rate of the supermask $S^T_l$,~\ie $sum(S^T_l) = k$. For instance, if the pruning-rate is $50\%$, then $k=\frac{|W_l|}{2}$. 

%where $D$ is a sampling distribution. For simplicity, our $D$ is a uniform categorical distribution over the $k$-weights inside $W^ \star_l$. The sampling distribution simulates the crossover operation in a genetic algorithm. We re-initialize all the network's layers using~\autoref{eq:transfer_fit_weights}. Then, we  re-enter the task phase. The bias terms are trained during the task-phase and frozen during the mask-phase. We re-initialize the bias of the next generation using the exact previous generation's bias. 


\begin{comment}
	\begin{figure}[t]
	\centering
	\scriptsize
	%	\begin{table}
	\renewcommand{\arraystretch}{1.5}
	\begin{tabular}{ c c c}
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{ |c| c| c| }
	\hline
	\cellcolor{gray!70}-1  & \cellcolor{gray!50}0 & \cellcolor{gray!30}1 \\ 	\hline
	\cellcolor{gray!90}-2   & \cellcolor{gray!50}0 & \cellcolor{gray!10}2 \\  	\hline
	\cellcolor{gray!70}-1  & \cellcolor{gray!50}0 & \cellcolor{gray!30}1  \\	\hline
	\end{tabular} & 
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{ |c| c| c| } 
	\hline
	\cellcolor{gray!70}-1& \cellcolor{gray!90}-2 & \cellcolor{gray!70}-1 \\ 	\hline
	\cellcolor{gray!50}0 & \cellcolor{gray!50}0 & \cellcolor{gray!50}0 \\  	\hline
	\cellcolor{gray!30}1& \cellcolor{gray!10}2 & \cellcolor{gray!30}1 \\ 	\hline
	\end{tabular} & 
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{ |c| c| c| } 
	\hline
	\cellcolor{gray!50}0& \cellcolor{gray!70}-1 & \cellcolor{gray!90}-2  \\ 	\hline
	\cellcolor{gray!30}1 & \cellcolor{gray!50}0 & \cellcolor{gray!70}-1 \\  	\hline
	\cellcolor{gray!10}2& \cellcolor{gray!30}1 & \cellcolor{gray!50}0 \\ 	\hline
	\end{tabular} 
	\\
	Vertical & Horizontal & Diagonal\\
	
	\end{tabular}
	%	\end{table}
	\caption{Sobel filter re-arrangement detect edges with different angles.}
	\label{fig:sobel_filter}
	\end{figure}
\end{comment}


%\autoref{fig:sobel_filter} illustrate the intuition behind the sampling formulation~(\autoref{eq:transfer_fit_weights}). Given a fit-filter (\eg vertical Sobel-filter), other fit-filters (\eg horizontal) are permutations of the original filter's values. \autoref{eq:transfer_fit_weights} is formulated not to sample a conv-filter as a unit but independent weights. This promotes KE for a large spectrum of neural layers. In addition, \autoref{eq:transfer_fit_weights} promotes fit-weights that are valuable across filters (\eg Sobel and Prewitt). 

\begin{algorithm}[t]
%	\scriptsize
	\SetAlgoLined
	\KwResult{A trained network $N$ with popup scores $S$}
	\BlankLine
	$W,F,B,BN,S$ are initialized randomly\;
	\For{generation $i$ \KwTo $G$}{
		freeze $S$\;
		Train 	$N$ on task $T$\tcp*{\text{Update} $W,B,BN,F$} 
		freeze  ${W,B,BN,F}$\;
		unfreeze $S$\;
		Find $H^\triangle$ using conv-popup \tcp*{\text{Update} $S$} 
		unfreeze ${W,B,BN,F}$\;
		\For{layer $l=0$ \KwTo $L$}{
			Update $W_l/B_l/F_l$ using~\autoref{eq:transfer_fit_hypothesis}
		}
	}
	\caption{Task-Mask algorithm trains a network $N$ with $L$ layers for $G$ generations on a supervised task $T$; The network $N$ has weights $W$, convolutional filters $F$, bias $B$, popup scores $S$, and batch norm parameters $BN$.}
	\label{Algo:task_mask}
\end{algorithm}
